LICORICE: Label-Efficient Concept-Based Interpretable Reinforcement Learning

Recent advances in reinforcement learning (RL) have predominantly leveraged neural network policies for decision-making, yet these models often lack interpretability, posing challenges for stakeholder comprehension and trust. Concept bottleneck models offer an interpretable alternative by integrating human-understandable concepts into policies. However, prior work assumes that concept annotations are readily available during training. For RL, this requirement poses a significant limitation: it necessitates continuous real-time concept annotation, which either places an impractical burden on human annotators or incurs substantial costs in API queries and inference time when employing automated labeling methods. To overcome this limitation, we introduce a novel training scheme that enables RL agents to efficiently learn a concept-based policy by only querying annotators to label a small set of data. Our algorithm, LICORICE, involves three main contributions: interleaving concept learning and RL training, using an ensemble to actively select informative data points for labeling, and decorrelating the concept data. We show how LICORICE reduces human labeling efforts to 500 or fewer concept labels in three environments, and 5000 or fewer in two more complex environments, all at no cost to performance. We also explore the use of VLMs as automated concept annotators, finding them effective in some cases but imperfect in others. Our work significantly reduces the annotation burden for interpretable RL, making it more practical for real-world applications that necessitate transparency.

==> sections/scratch.tex <==
also put the imitation learning possibility

\smnote{Goals:
\begin{itemize}
    \item Produce useful interpretable world models for reinforcement learning.
\end{itemize}
}


\smnote{Challenges in learning factored models:
\begin{enumerate}
    \item Assume that the encoder $e_\phi(\cdot)$ can produce a factorized representation. 
    When decoding the latent variable, the decoder $d_\phi(\cdot)$ may undo the factorization. 
    \smcomment{I am not super clear on why this happens -- some more explanation would be very useful!}
    \item The latent variable is typically uninterpretable, which makes it difficult to verify that the learned model indeed learns critical, human-interpretable factors.
\end{enumerate}
}

\smnote{Potential research questions:
\begin{itemize}
    \item Does learning ``aligned'' world models (e.g., through shared concept bottlenecks or language grounding) facilitate better coordination between AI and/or human agents? 
    Potential contribution: include concept bottlenecks~\citep{koh2020concept} for both the encoder and decoder, such that each component of the world model is bottlenecked by these concepts. 
    See \Cref{sec:method} for some more details of what this could look like.
    \item Does learning interpretable world models permit more explanations? E.g., concept bottlnecks allow different types of interpretable counterfactual explanaitons in the world model.
\end{itemize}
}


\smnote{
Note the assumptions here are that 1) we get access to a lot of labeled data at the beginning, 2) we have concept representations in the form of binary representations, 3) that there is no spatial or other semantics that may induce different classifications (mapping of c to y is basically the task, use simple concepts to produce label). 
in theory, we could have x to c to y to a so that we can understand what produces a higher-level concept while still taking actions with fewer inputs. also another thing could be to decide when to use an aggregate concept and when to use a more basic concept (like maybe just the presence of black is sufficient, we don't need to know which type of object, but maybe a blue door is meaningful but a blue chair is not). 
}

\smnote{Continuing with the above, the next step may be to try to have some sort of sparse concept dependency for interpretability (intuition: people may not understand actions as a function of $10$ concepts very well, but could understand $2-3$). Another direction is: if concepts frequently occur together, they may be better understood under its own name.}


\subsection{VAE}
The original world models paper~\citep{ha2018world} includes a simple pipeline for producing a model-based reinforcement learning agent for a single agent setting.
This pipeline includes a VAE~\citep{kingma2013auto} for the world model component.

Outside of the realm of model-based reinforcement learning, researchers proposed $\beta$-VAE~\citep{higgins2017beta} for unsupervised learning of the interpretable factorized representations of the independent generative factors of the world.
They assume that there exist two sets of data generative factors: conditionally independent ones $v \in \mathbb{R}^K$ and conditionally dependent ones $w \in \mathbb{R}^H$. 
They assume that the images $x$ are generated by the world simulator using the ground-truth generative factors $p(x|v,w)=\text{Sim}(v,w)$.
Note that they do not assume these factors to be known; instead, they want to discover them. 
They write the $\beta$-VAE formulation as: $$\mathcal{F}(\theta, \phi, \beta; x,z) \geq \mathcal{L}(\theta, \phi; x, z, \beta) = \mathbb{E}_{q_\phi(z|x)} [\log p_\theta(x|z)] -\beta D_{KL}(q_\phi(z|x)||p(z)).$$
Here, $\beta$ is a regularization coefficient that constrains the capacity of the latent information channel $z$ and puts independence pressure on the learned posterior $q_\phi(z|x)$ due to the isotropic Gaussian prior $p(z)$.
Note that $\beta=1$ is simply the original VAE formulation; to learn disentangled representations, we must set $\beta > 1$ to limit the capacity of $z$.
The tricky part of this formulation is that we must strike the right balance between information preservation (reconstruction cost) and capacity restriction through setting $\beta > 1$.

On the other hand, concept bottleneck networks involve predicting a target $y \in \mathbb{R}$ from input $x\in\mathbb{R}^d$.
The training points consist of $\{(x^{(i)}, y^{(i)}, c^{(i)}\}^n_{i=1}$, where $c \in \mathbb{R}^k$ is a vector of $k$ concepts.
Bottleneck models take the form $f(g(x))$, where $g : \mathbb{R}^d \rightarrow \mathbb{R}^k$ maps $x$ to the concept space and $f : \mathbb{R}^k \rightarrow \mathbb{R}$ maps concepts into a final prediction.

In a VAE, we have a probabilistic encoder $q_\phi(z|x)$ that produces a distribution over the possible values of the code $z$ from which the datapoint $x$ could have been generated.
We also have a probabilistic decoder $p_\theta(x|z)$ that produces a distribution over the possible values of $x$ given a code $z$. 
Because we are only interested in learning from the latent space, we want a concept-bottleneck encoder.
In other words, we want the encoder to produce a distribution over the possible values of the code $z$ with respect to a set of concepts $c$.
We now have the additional $\hat{g}$ to learn, such that $\hat{g} =\mathrm{argmin}_g\sum_{i,j} L_{C_j}(g_j(x^{(i)}); c_j^{(i)})$.
Here, $L_{C_j}: \mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}_{+}$ is a loss function that measures the discrepancy between the predicted and true $j$-th concept.
We derive the ELBO loss for the sequential bottleneck here.

We will now derive the VAE objective with respect to these concept bottlenecks. 
Note that the lower bound $\mathcal{L}$ is a surrogate for our distribution of interest $p(g(x))$, where $g(x)$ is again our function mapping $x$ to the concept space.
Rewriting the $\beta$-VAE formulation, we have:
$$\mathcal{F}(\theta, \phi, \beta; x,z) \geq \mathcal{L}(\theta, \phi; x, z, \beta) = \mathbb{E}_{q_\phi(\hat{g}(z)|x)} [\log p_\theta(\hat{g}(x)|z)] -\beta D_{KL}(q_\phi(\hat{g}(z)|x)||p(\hat{g}(z))).$$
Since the sequential bottleneck first learns $\hat{g}$, our loss remains unchanged. 
\smnote{we may want to change this -- need to check the bottleneck paper more carefully to see which formulation they recommend. also should check the vae objective more carefully. TODO check the gen models paper and use their formulation.}

\section{Dreamer Scratch}

Another direction we can go is the following. 
We want to propogate the learned concepts through the entire Dreamer architecture. 
That means that we want $z_t$ and $h_t$ to both be interpretable.
For $z_t$, this is straightforward if we can get concept labels for $h_t$, as we already have concept labels $c_t$ for $x_t$.
\smnote{
Given that $f_\phi$ is implemented as an RNN with multiple inputs, we must have associated concept data with those inputs. 
In particular, we need to encode the output from each time step of the RNN $(h_t)$ through the concept bottleneck $g$ to map the hidden states to a concept space. 
We proposed to build off of work on transforming RNNs to finite-state representations known as a Moore Machine through Quantized Bottleneck Network (QBN) insertion.
(We note that in previous work the idea is to learn these embeddings after training an RNN, so we either need to follow the assumptions here or come up with a new idea for training.) 
The idea here is to instantiate the QBN as an autoencoder that constrains the latent representation between the encoder and decoder to be composed of $k$-level activation units. 
Therefore, the QBN output is $b(x)=D(\mathrm{quantize}(E(x)).$
Here, we can assume the quantization is binary, representing the presence or absence of a concept. 
Since the quantize function is now non-differentiable, straight-through estimators of the gradient are necessary to use backpropagation. 
Specifically, treating the quantize function as the identity function during backpropagation. 
Considerations here include: do we insert the concept bottlenecks during this training part? 
Or is it useful to get this quantization, then insert concept bottlenecks and fine tune.
The benefit of the latter is that the quantization can help tell us which parts of the history actually are used, which means that the hidden state is a function of those specific previous observations, narrowing down the concepts needed for prediction. 
My understanding of what is necessary here is a little fuzzy. 
}

One caveat is that concept bottleneck networks require the recognition of these concepts ahead of time to inject them into the network.
Another caveat is that the images need to be labeled with these concepts, which makes things challenging. 
Main question is how do we obtain densely labeled concept data for reinforcement learning?
Answer: use LLMs to help provide additional potential concept labels given an image. 
